Timed Partial Order Inference Algorithm

In this work, we propose the model of timed partial orders (TPOs) for specifying workflow schedules, especially for modeling manufacturing processes. TPOs integrate partial orders over events in a workflow, specifying ``happens-before'' relations, with timing constraints specified using guards and resets on clocks -- an idea borrowed from timed-automata specifications. TPOs naturally allow us to capture event ordering, along with a restricted but useful class of timing relationships. Next, we consider the problem of mining TPO schedules from workflow logs, which include events along with their time stamps. We demonstrate a relationship between formulating TPOs and the graph-coloring problem, and present an algorithm for learning TPOs with correctness guarantees. We demonstrate our approach on synthetic datasets, including two datasets inspired by real-life applications of aircraft turnaround and gameplay videos of the Overcooked computer game. Our TPO mining algorithm can infer TPOs involving hundreds of events from thousands of data-points within a few seconds. We show that the resulting TPOs provide useful insights into the dependencies and timing constraints for workflows.

==> sections/ClockAssigningAlgorithm.tex <==
\begin{algorithm}[t]
\caption{\textsc{AssignClocks}}
\label{alg:ClockAssignmingAlgorithm}
\textbf{Input}: Partial Order Graph $\APO$, Time Constraints $TC$, Backward Partial Order $B$\\
\textbf{Output}: A Timed Partial Order Graph $\ATPO$

\begin{algorithmic}[1]
\setcounter{ALC@unique}{0}
\STATE Add a dummy initial node and edges to $\APO$ and $TC$
\STATE Initialize ClocksInUse $C$
\STATE Initialize ResetClocks $R$, EdgeClocks $E$
\STATE Initialize queue $Q$ with the dummy initial node
\WHILE{$Q$ is not empty}{
    \STATE $n \leftarrow Q.pop()$
    \IF{$\exists c\in C$ s.t. nodes that use $c$ are in $B(n)$} 
        \STATE $reset \leftarrow c$
    \ELSE
        \STATE Create a new clock $reset$
    \ENDIF
    
    \STATE Register $reset$ as a node $n$'s reset clock in $R$ 
    \STATE Register $reset$ as a $n$'s target node clocks in $E$
    
    \STATE Add all successors of $n$ that are not yet visited to $Q$
}
\ENDWHILE
\RETURN{Label $\APO$ with clocks and its bounds based on $TC$, $R$, $E$}
\end{algorithmic}
\end{algorithm}



==> sections/PartialOrderIdentificationAlgorithm.tex <==
\begin{algorithm}[t]
\caption{\textsc{identifyPartialOrderGraph}}
\label{alg:PartialOrderIdentification}
\textbf{Input}: Timed Traces $\TimedTraces$\\
\textbf{Output}: A Partial Order Graph $\APO$

\begin{algorithmic}[1]
\STATE Initialize Forwards $F$
\STATE Initialize Backwards $B$
\FOR{$\timedtrace \in \TimedTraces$}
    \FOR{$i \in [0, \ldots, |\timedtrace|-1]$}
        \STATE $\event_i \leftarrow \timedtrace[i]$
        \STATE Add events to Forwards $F[\event_i].add(\timedtrace[i+1:])$
        \STATE Add events to Backwards $B[\event_i].add(\timedtrace[:i])$
    \ENDFOR
\ENDFOR
\FOR{$\event_i \in \events$}
    \STATE $\PO \leftarrow F[\event_i] - B[\event_i]$
\ENDFOR
\STATE $\APO = \textsc{convertToGraph}(\PO)$
\STATE $\APO = \textsc{transitiveReduce}(\APO)$
\RETURN $\APO$
\end{algorithmic}
\end{algorithm}



==> sections/TimedPartialOrderInfereceAlgorithm.tex <==
\begin{algorithm}[t]
\caption{\textsc{TimedPartialOrderInference}}
\label{alg:TimedPartialOrderInfernece}
\textbf{Input}: Timed Traces $\TimedTraces$, Threshold $\gamma$\\
\textbf{Output}: A Timed Partial Order Graph $\ATPO$

\begin{algorithmic}[1]
\setcounter{ALC@unique}{0}
\STATE $\APO = \textsc{identifyPartialOrderGraph}(\TimedTraces)$
\STATE $TC \leftarrow \textsc{constructLPConsraints}(\TimedTraces)$ \label{line:construct_lp}
\STATE Initialize a time constraint variable $tc$
\STATE Initialize the time constraints list $TC'$
\WHILE{$tc$ is not None}{
    \STATE $tc \leftarrow \textsc{pickConstraint}(TC)$ \label{line:pickConstraint}
    
    \STATE $redundant = \textsc{checkIfRedundant}(TC, tc, \gamma)$ \label{line:checkIfRedundant}
    
    \IF{not $redundant$}
        \STATE Append $tc$ to $TC'$
    \ENDIF
    
    % \STATE $redundant = \textsc{removeConstraint}(C, c)$
    \STATE $\textsc{removeConstraint}(C, c, redundant)$  \label{line:removeConstraint}
}
\ENDWHILE
\STATE $\ATPO \leftarrow \textsc{AssignClocks}(\APO, C')$
\RETURN{$\ATPO$}
\end{algorithmic}
\end{algorithm}


